When Calibration Data Matter in Sub-4-Bit Language Model Quantization

Low-bit post-training quantization reduces language-model memory but can sharply degrade downstream task accuracy. Calibration usually relies on generic text, but when task-informed data recover accuracy and which quantizers benefit remain poorly understood. We introduce FragCal-DC, which supplements generic text with training documents from task families with low retention of full-precision accuracy in a two-bit scan. We use a two- to four-bit sweep to locate functional regimes and four-seed calibration comparisons to evaluate six data-dependent methods across six dense models (1.7B-8B) and ten tasks. At their lowest tested functional bit widths, iterative SignRound V2 and OmniQuant improve at two bits, whereas single-pass GPTQ and AWQ show small mean responses at three bits. At two bits, SignRound V2 gains 1.83 percentage points in mean ten-task accuracy over generic-text calibration across six models. At 70 billion parameters, GPTQ and SignRound V2 both improve at two bits, with functional generic-calibration baselines. For two-bit SignRound V2, task-level controls show that recovery concentrates on families included in calibration, while incorrect answer designations retain about 90% of the mean accuracy gain. Changes in reconstruction error do not consistently track accuracy gains. These findings support task-informed calibration as a design principle for preserving downstream accuracy in low-bit quantization.

==> generated/alternative_rows.tex <==
Diversity-DC & $+2.01$ & $[+0.08,+3.94]$ & 4/5 \\
LSA-DC & $+1.11$ & $[-0.17,+2.38]$ & 4/5 \\
ArXiv-OOD & $+2.55$ & $[+1.32,+3.77]$ & 5/5 \\


==> generated/answer_model_rows.tex <==
Llama-2-7B & $+1.31$ & $+0.59$ & $+1.40$ & 107.0\% \\
Mistral-7B & $+2.36$ & $+1.45$ & $+2.32$ & 98.3\% \\
Q2.5-7B-Inst & $+0.54$ & $+0.39$ & $+0.30$ & 56.2\% \\
Qwen3-1.7B & $+2.31$ & $+1.01$ & $+1.83$ & 79.0\% \\
Qwen3-8B & $+1.50$ & $+0.95$ & $+1.37$ & 91.2\% \\
Phi-3-mini & +2.97 & +2.12 & +2.69 & 91\% \\
\midrule
\textbf{Six-model mean} & \textbf{+1.83} & \textbf{+1.09} & \textbf{+1.65} & \textbf{90\%} \\


==> generated/answer_summary_rows.tex <==
\spclass~RTN-opt FragCal & 0.3843 & $-0.04$ & $[-0.35,+0.28]$ & --- \\
\spclass~RTN-opt Pile-200 & 0.3846 & --- & --- & --- \\
\midrule
\itclass~SR-V2 correct & 0.5551 & $+1.60$ & $[+0.66,+2.55]$ & 100.0\% \\
\itclass~SR-V2 wrong & 0.5535 & $+1.44$ & $[+0.52,+2.37]$ & 90.0\% \\
\itclass~SR-V2 no designation & 0.5478 & $+0.88$ & $[+0.38,+1.39]$ & 54.9\% \\
\itclass~SR-V2 Pile-200 & 0.5390 & --- & --- & --- \\


==> generated/baseline_mean_rows.tex <==
W2G128 & 0.643 & 0.314\,\xmark & 0.386\,\cmark & 0.308\,\xmark & 0.306\,\xmark & 0.388\,\cmark & 0.536\,\cmark & 0.596\,\cmark \\
W3G128 & 0.643 & 0.550\,\cmark & 0.594\,\cmark & 0.603\,\cmark & 0.576\,\cmark & 0.604\,\cmark & 0.623\,$\uparrow$ & --- \\
W4G128 & 0.643 & 0.627\,$\uparrow$ & 0.631\,$\uparrow$ & 0.635\,$\uparrow$ & 0.638\,$\uparrow$ & 0.634\,$\uparrow$ & 0.633\,$\uparrow$ & --- \\


==> generated/baseline_w2_rows.tex <==
Qwen3-1.7B & .559 & .303 & .313 & .320 & .306 & .363 & .428 & .512 \\
Llama-2-7B & .608 & .321 & .413 & .294 & .313 & .343 & .528 & .571 \\
Mistral-7B & .664 & .352 & .447 & .298 & .306 & .301 & .564 & .620 \\
Q2.5-7B-Inst & .692 & .311 & .367 & .298 & .311 & .477 & .605 & .620 \\
Qwen3-8B & .662 & .290 & .385 & .319 & .302 & .455 & .572 & .627 \\
Phi-3 & .672 & .304 & .389 & .318 & .298 & .389 & .522 & .628 \\


==> generated/baseline_w3_rows.tex <==
Qwen3-1.7B & .559 & .417 & .455 & .488 & .443 & .507 & .527 \\
Llama-2-7B & .608 & .580 & .589 & .577 & .570 & .583 & .590 \\
Mistral-7B & .664 & .623 & .634 & .634 & .620 & .625 & .645 \\
Q2.5-7B-Inst & .692 & .615 & .644 & .667 & .635 & .658 & .675 \\
Qwen3-8B & .662 & .570 & .623 & .623 & .605 & .631 & .649 \\
Phi-3 & .672 & .494 & .618 & .631 & .583 & .622 & .649 \\


==> generated/baseline_w4_rows.tex <==
Qwen3-1.7B & .559 & .524 & .535 & .547 & .541 & .548 \\
Llama-2-7B & .608 & .603 & .603 & .606 & ---$^\dagger$ & .603 \\
Mistral-7B & .664 & .653 & .654 & .659 & .656 & .654 \\
Q2.5-7B-Inst & .692 & .678 & .676 & .682 & .680 & .682 \\
Qwen3-8B & .662 & .648 & .649 & .652 & .656 & .654 \\
Phi-3 & .672 & .653 & .668 & .664 & .655 & .664 \\


==> generated/cross_model_rows.tex <==
\spclass~RTN-opt & Llama-2-7B & W2G128 & Pile-200 & 0.4130 & 0.4119 & $-0.12$ & $-0.6$ \\
\spclass~RTN-opt & Llama-2-7B & W3G128 & Pile-200 & 0.5886 & 0.5883 & $-0.02$ & $-1.1$ \\
\spclass~RTN-opt & Llama-2-7B & W4G128 & Pile-200 & 0.6032 & 0.6033 & $+0.01$ & $+1.8$ \\
\spclass~RTN-opt & Mistral-7B & W2G128 & Pile-200 & 0.4423 & 0.4444 & $+0.21$ & $+1.0$ \\
\spclass~RTN-opt & Mistral-7B & W3G128 & Pile-200 & 0.6346 & 0.6342 & $-0.05$ & $-1.6$ \\
\spclass~RTN-opt & Mistral-7B & W4G128 & Pile-200 & 0.6584 & 0.6586 & $+0.03$ & $+5.1$ \\
\spclass~RTN-opt & Phi-3-mini & W2G128 & Pile-200 & 0.3885 & 0.3872 & $-0.13$ & $-0.4$ \\
\spclass~RTN-opt & Phi-3-mini & W3G128 & Pile-200 & 0.6179 & 0.6211 & $+0.32$ & $+5.9$ \\
\spclass~RTN-opt & Phi-3-mini & W4G128 & Pile-200 & 0.6673 & 0.6668 & $-0.05$ & $-9.3$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & W2G128 & Pile-200 & 0.3706 & 0.3690 & $-0.16$ & $-0.5$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & W3G128 & Pile-200 & 0.6436 & 0.6443 & $+0.08$ & $+1.6$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & W4G128 & Pile-200 & 0.6813 & 0.6804 & $-0.09$ & $-9.0$ \\
\spclass~RTN-opt & Qwen3-1.7B & W2G128 & Pile-200 & 0.3105 & 0.3070 & $-0.35$ & $-1.4$ \\
\spclass~RTN-opt & Qwen3-1.7B & W3G128 & Pile-200 & 0.4580 & 0.4553 & $-0.26$ & $-2.6$ \\
\spclass~RTN-opt & Qwen3-1.7B & W4G128 & Pile-200 & 0.5358 & 0.5354 & $-0.04$ & $-1.7$ \\
\spclass~RTN-opt & Qwen3-8B & W2G128 & Pile-200 & 0.3867 & 0.3890 & $+0.23$ & $+0.8$ \\
\spclass~RTN-opt & Qwen3-8B & W3G128 & Pile-200 & 0.6224 & 0.6204 & $-0.19$ & $-4.8$ \\
\spclass~RTN-opt & Qwen3-8B & W4G128 & Pile-200 & 0.6492 & 0.6493 & $+0.01$ & $+0.4$ \\
\spclass~AWQ & Llama-2-7B & W2G128 & Pile-200 & 0.2946 & 0.2938 & $-0.07$ & $-0.2$ \\
\spclass~AWQ & Llama-2-7B & W3G128 & Pile-200 & 0.5819 & 0.5826 & $+0.07$ & $+2.7$ \\
\spclass~AWQ & Llama-2-7B & W4G128 & Pile-200 & 0.6056 & 0.6052 & $-0.05$ & $-21.0$ \\
\spclass~AWQ & Mistral-7B & W2G128 & Pile-200 & 0.2987 & 0.2990 & $+0.03$ & $+0.1$ \\
\spclass~AWQ & Mistral-7B & W3G128 & Pile-200 & 0.6365 & 0.6391 & $+0.25$ & $+9.1$ \\
\spclass~AWQ & Mistral-7B & W4G128 & Pile-200 & 0.6571 & 0.6572 & $+0.01$ & $+1.0$ \\
\spclass~AWQ & Phi-3-mini & W2G128 & Pile-200 & 0.3173 & 0.3185 & $+0.12$ & $+0.3$ \\
\spclass~AWQ & Phi-3-mini & W3G128 & Pile-200 & 0.6334 & 0.6349 & $+0.14$ & $+3.7$ \\
\spclass~AWQ & Phi-3-mini & W4G128 & Pile-200 & 0.6639 & 0.6660 & $+0.21$ & $+25.5$ \\
\spclass~AWQ & Q2.5-7B-Inst & W2G128 & Pile-200 & 0.2976 & 0.2967 & $-0.09$ & $-0.2$ \\
\spclass~AWQ & Q2.5-7B-Inst & W3G128 & Pile-200 & 0.6630 & 0.6581 & $-0.49$ & $-17.3$ \\
\spclass~AWQ & Q2.5-7B-Inst & W4G128 & Pile-200 & 0.6842 & 0.6842 & $+0.00$ & $+0.3$ \\
\spclass~AWQ & Qwen3-1.7B & W2G128 & Pile-200 & 0.3196 & 0.3199 & $+0.04$ & $+0.2$ \\
\spclass~AWQ & Qwen3-1.7B & W3G128 & Pile-200 & 0.4899 & 0.4863 & $-0.35$ & $-5.1$ \\
\spclass~AWQ & Qwen3-1.7B & W4G128 & Pile-200 & 0.5486 & 0.5432 & $-0.54$ & $-54.0$ \\
\spclass~AWQ & Qwen3-8B & W2G128 & Pile-200 & 0.3209 & 0.3216 & $+0.07$ & $+0.2$ \\
\spclass~AWQ & Qwen3-8B & W3G128 & Pile-200 & 0.6270 & 0.6285 & $+0.15$ & $+4.3$ \\
\spclass~AWQ & Qwen3-8B & W4G128 & Pile-200 & 0.6530 & 0.6547 & $+0.18$ & $+19.1$ \\
\spclass~GPTQ & Llama-2-7B & W2G128 & Pile-200 & 0.3187 & 0.3264 & $+0.77$ & $+2.7$ \\
\spclass~GPTQ & Llama-2-7B & W3G128 & Pile-200 & 0.5743 & 0.5718 & $-0.25$ & $-7.5$ \\
\spclass~GPTQ & Llama-2-7B & W4G128 & Pile-200 & 0.6018 & 0.5946 & $-0.72$ & $-118.6$ \\
\spclass~GPTQ & Mistral-7B & W2G128 & Pile-200 & 0.3101 & 0.2960 & $-1.41$ & $-4.0$ \\
\spclass~GPTQ & Mistral-7B & W3G128 & Pile-200 & 0.6192 & 0.6094 & $-0.98$ & $-21.9$ \\
\spclass~GPTQ & Mistral-7B & W4G128 & Pile-200 & 0.6549 & 0.6557 & $+0.08$ & $+8.9$ \\
\spclass~GPTQ & Phi-3-mini & W2G128 & Pile-200 & 0.2986 & 0.3018 & $+0.32$ & $+0.8$ \\
\spclass~GPTQ & Phi-3-mini & W3G128 & Pile-200 & 0.5789 & 0.5909 & $+1.21$ & $+12.9$ \\
\spclass~GPTQ & Phi-3-mini & W4G128 & Pile-200 & 0.6554 & 0.6564 & $+0.11$ & $+6.3$ \\
\spclass~GPTQ & Q2.5-7B-Inst & W2G128 & Pile-200 & 0.3127 & 0.3148 & $+0.21$ & $+0.5$ \\
\spclass~GPTQ & Q2.5-7B-Inst & W3G128 & Pile-200 & 0.6309 & 0.6372 & $+0.63$ & $+10.5$ \\
\spclass~GPTQ & Q2.5-7B-Inst & W4G128 & Pile-200 & 0.6829 & 0.6853 & $+0.24$ & $+27.8$ \\
\spclass~GPTQ & Qwen3-1.7B & W2G128 & Pile-200 & 0.3052 & 0.2992 & $-0.60$ & $-2.4$ \\
\spclass~GPTQ & Qwen3-1.7B & W3G128 & Pile-200 & 0.4475 & 0.4391 & $-0.84$ & $-7.5$ \\
\spclass~GPTQ & Qwen3-1.7B & W4G128 & Pile-200 & 0.5304 & 0.5275 & $-0.29$ & $-10.3$ \\
\spclass~GPTQ & Qwen3-8B & W2G128 & Pile-200 & 0.3169 & 0.2976 & $-1.93$ & $-5.6$ \\
\spclass~GPTQ & Qwen3-8B & W3G128 & Pile-200 & 0.5974 & 0.6136 & $+1.62$ & $+25.0$ \\
\spclass~GPTQ & Qwen3-8B & W4G128 & Pile-200 & 0.6531 & 0.6545 & $+0.14$ & $+15.1$ \\
\itclass~OmniQuant & Llama-2-7B & W2G128 & Pile-200 & 0.3820 & 0.3947 & $+1.27$ & $+5.6$ \\
\itclass~OmniQuant & Llama-2-7B & W3G128 & Pile-200 & 0.5801 & 0.5834 & $+0.33$ & $+11.8$ \\
\itclass~OmniQuant & Llama-2-7B & W4G128 & Pile-200 & 0.6030 & 0.6021 & $-0.08$ & $-17.5$ \\
\itclass~OmniQuant & Mistral-7B & W2G128 & Pile-200 & 0.3201 & 0.3031 & $-1.70$ & $-4.9$ \\
\itclass~OmniQuant & Mistral-7B & W3G128 & Pile-200 & 0.6247 & 0.6250 & $+0.03$ & $+0.9$ \\
\itclass~OmniQuant & Mistral-7B & W4G128 & Pile-200 & 0.6536 & 0.6537 & $+0.01$ & $+1.1$ \\
\itclass~OmniQuant & Phi-3-mini & W2G128 & Pile-200 & 0.3903 & 0.4090 & $+1.87$ & $+6.6$ \\
\itclass~OmniQuant & Phi-3-mini & W3G128 & Pile-200 & 0.6193 & 0.6228 & $+0.35$ & $+6.6$ \\
\itclass~OmniQuant & Phi-3-mini & W4G128 & Pile-200 & 0.6620 & 0.6615 & $-0.06$ & $-5.5$ \\
\itclass~OmniQuant & Q2.5-7B-Inst & W2G128 & Pile-200 & 0.5147 & 0.5300 & $+1.53$ & $+8.7$ \\
\itclass~OmniQuant & Q2.5-7B-Inst & W3G128 & Pile-200 & 0.6605 & 0.6613 & $+0.08$ & $+2.4$ \\
\itclass~OmniQuant & Q2.5-7B-Inst & W4G128 & Pile-200 & 0.6837 & 0.6835 & $-0.03$ & $-3.7$ \\
\itclass~OmniQuant & Qwen3-1.7B & W2G128 & Pile-200 & 0.3658 & 0.3847 & $+1.89$ & $+9.8$ \\
\itclass~OmniQuant & Qwen3-1.7B & W3G128 & Pile-200 & 0.5156 & 0.5087 & $-0.69$ & $-16.0$ \\
\itclass~OmniQuant & Qwen3-1.7B & W4G128 & Pile-200 & 0.5497 & 0.5475 & $-0.22$ & $-24.7$ \\
\itclass~OmniQuant & Qwen3-8B & W2G128 & Pile-200 & 0.4598 & 0.4830 & $+2.32$ & $+11.5$ \\
\itclass~OmniQuant & Qwen3-8B & W3G128 & Pile-200 & 0.6314 & 0.6274 & $-0.41$ & $-13.2$ \\
\itclass~OmniQuant & Qwen3-8B & W4G128 & Pile-200 & 0.6541 & 0.6529 & $-0.11$ & $-14.0$ \\
\itclass~SR-V2 & Llama-2-7B & W2G128 & Pile-200 & 0.5224 & 0.5355 & $+1.31$ & $+15.3$ \\
\itclass~SR-V2 & Llama-2-7B & W3G128 & Pile-200 & 0.5840 & 0.5943 & $+1.02$ & $+42.9$ \\
\itclass~SR-V2 & Llama-2-7B & W4G128 & Pile-200 & 0.6067 & 0.6050 & $-0.18$ & $-155.4$ \\
\itclass~SR-V2 & Mistral-7B & W2G128 & Pile-200 & 0.5653 & 0.5889 & $+2.36$ & $+23.9$ \\
\itclass~SR-V2 & Mistral-7B & W3G128 & Pile-200 & 0.6452 & 0.6480 & $+0.28$ & $+14.7$ \\
\itclass~SR-V2 & Mistral-7B & W4G128 & Pile-200 & 0.6583 & 0.6595 & $+0.12$ & $+20.2$ \\
\itclass~SR-V2 & Phi-3-mini & W2G128 & Pile-200 & 0.5252 & 0.5549 & $+2.97$ & $+20.2$ \\
\itclass~SR-V2 & Phi-3-mini & W3G128 & Pile-200 & 0.6460 & 0.6511 & $+0.51$ & $+19.6$ \\
\itclass~SR-V2 & Phi-3-mini & W4G128 & Pile-200 & 0.6688 & 0.6685 & $-0.04$ & $-11.3$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & W2G128 & Pile-200 & 0.6018 & 0.6072 & $+0.54$ & $+6.0$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & W3G128 & Pile-200 & 0.6723 & 0.6729 & $+0.06$ & $+2.9$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & W4G128 & Pile-200 & 0.6858 & 0.6863 & $+0.05$ & $+8.4$ \\
\itclass~SR-V2 & Qwen3-1.7B & W2G128 & Pile-200 & 0.4349 & 0.4580 & $+2.31$ & $+18.7$ \\
\itclass~SR-V2 & Qwen3-1.7B & W3G128 & Pile-200 & 0.5317 & 0.5363 & $+0.46$ & $+17.0$ \\
\itclass~SR-V2 & Qwen3-1.7B & W4G128 & Pile-200 & 0.5540 & 0.5537 & $-0.03$ & $-6.6$ \\
\itclass~SR-V2 & Qwen3-8B & W2G128 & Pile-200 & 0.5708 & 0.5858 & $+1.50$ & $+16.4$ \\
\itclass~SR-V2 & Qwen3-8B & W3G128 & Pile-200 & 0.6518 & 0.6502 & $-0.15$ & $-14.8$ \\
\itclass~SR-V2 & Qwen3-8B & W4G128 & Pile-200 & 0.6593 & 0.6606 & $+0.13$ & $+45.8$ \\
\itclass~AQLM & Llama-2-7B & W2-eq. & Pile-200 & 0.5675 & 0.5733 & $+0.58$ & $+14.3$ \\
\itclass~AQLM & Mistral-7B & W2-eq. & Pile-200 & 0.6250 & 0.6371 & $+1.21$ & $+30.8$ \\
\itclass~AQLM & Phi-3-mini & W2-eq. & Pile-200 & 0.6235 & 0.6334 & $+0.98$ & $+20.2$ \\
\itclass~AQLM & Q2.5-7B-Inst & W2-eq. & Pile-200 & 0.5946 & 0.5875 & $-0.71$ & $-7.4$ \\
\itclass~AQLM & Qwen3-1.7B & W2-eq. & Pile-200 & 0.5033 & 0.5209 & $+1.76$ & $+31.8$ \\
\itclass~AQLM & Qwen3-8B & W2-eq. & Pile-200 & 0.6299 & 0.6357 & $+0.59$ & $+18.2$ \\


==> generated/fp_task_rows.tex <==
ARC-C & .429 & .451 & .539 & .547 & .568 & .565 \\
ARC-E & .725 & .755 & .802 & .816 & .835 & .817 \\
BoolQ & .777 & .793 & .843 & .864 & .866 & .854 \\
HellaSwag & .604 & .762 & .812 & .805 & .750 & .775 \\
LAMBADA & .504 & .736 & .750 & .695 & .643 & .645 \\
MMLU & .554 & .417 & .600 & .717 & .730 & .699 \\
OpenBookQA & .362 & .442 & .460 & .486 & .416 & .476 \\
PIQA & .726 & .781 & .806 & .794 & .768 & .795 \\
TruthfulQA & .294 & .248 & .282 & .485 & .367 & .364 \\
WinoGrande & .612 & .693 & .748 & .707 & .678 & .732 \\
AVG & .559 & .608 & .664 & .692 & .662 & .672 \\


==> generated/historical_seed_gptq_rows.tex <==
Qwen3-1.7B & 0.4431 & 0.4479 & 0.4547 & 0.4401 & 0.4465 & 0.0056 & 1.25\% \\
Llama-2-7B & 0.5700 & 0.5710 & 0.5728 & 0.5694 & 0.5708 & 0.0013 & 0.22\% \\
Mistral-7B & 0.6201 & 0.6228 & 0.6251 & 0.6189 & 0.6217 & 0.0024 & 0.38\% \\
Q2.5-7B-Inst & 0.6345 & 0.6352 & 0.6378 & 0.6329 & 0.6351 & 0.0018 & 0.28\% \\
Qwen3-8B & 0.6053 & 0.6021 & 0.6085 & 0.6019 & 0.6045 & 0.0028 & 0.46\% \\
Phi-3 & 0.5829 & 0.5767 & 0.5799 & 0.5759 & 0.5788 & 0.0032 & 0.55\% \\


==> generated/historical_seed_oq_rows.tex <==
Qwen3-1.7B & .3658 & .0039 & 1.07\% & .0093 & .3847 & .0031 & 0.81\% & .0072 \\
Llama-2-7B & .3820 & .0061 & 1.60\% & .0141 & .3947 & .0049 & 1.24\% & .0117 \\
Mistral-7B$^{\dagger}$ & .3067 & .0005 & 0.17\% & .0010 & .3031 & .0042 & 1.39\% & .0084 \\
Q2.5-7B-Inst & .5147 & .0105 & 2.04\% & .0212 & .5300 & .0051 & 0.96\% & .0117 \\
Qwen3-8B & .4598 & .0022 & 0.48\% & .0047 & .4830 & .0013 & 0.27\% & .0032 \\
Phi-3 & .3903 & .0013 & 0.33\% & .0031 & .4090 & .0024 & 0.59\% & .0046 \\


==> generated/historical_seed_srv2_rows.tex <==
Qwen3-1.7B & 0.4552 & 0.4593 & 0.4622 & 0.4552 & 0.4580 & 0.0030 & 0.66\% \\
Llama-2-7B & 0.5355 & 0.5357 & 0.5404 & 0.5310 & 0.5356 & 0.0038 & 0.71\% \\
Mistral-7B & 0.5869 & 0.5880 & 0.5948 & 0.5857 & 0.5888 & 0.0041 & 0.70\% \\
Q2.5-7B-Inst & 0.6075 & 0.6078 & 0.6074 & 0.6060 & 0.6072 & 0.0007 & 0.12\% \\
Qwen3-8B & 0.5865 & 0.5867 & 0.5865 & 0.5834 & 0.5858 & 0.0014 & 0.24\% \\
Phi-3 & 0.5564 & 0.5535 & 0.5510 & 0.5586 & 0.5549 & 0.0033 & 0.59\% \\


==> generated/historical_volume_rows.tex <==
Q3-1.7B & +0.54pp & +0.32pp & $-$0.06pp \\
Llama-2-7B & $-$0.52pp & $-$0.43pp & +0.04pp \\
Mistral-7B & +0.17pp & +0.13pp & +0.15pp \\
Q2.5-7B-Inst & $-$0.33pp & $-$0.11pp & +0.03pp \\
Q3-8B & $-$0.12pp & +0.19pp & $-$0.04pp \\
Mean & $-0.05$ & $+0.02$ & $+0.02$ \\


==> generated/loss_summary_rows.tex <==
\spclass~AWQ & 6 & $+7.80$ & $-0.04$ & 4/6 \\
\spclass~GPTQ & 6 & $+3.90$ & $+0.23$ & 2/6 \\
\itclass~OmniQuant & 5 & $-0.22$ & $+1.78$ & 3/5 \\
\itclass~SR-V2 & 6 & $-5.12$ & $+1.83$ & 2/6 \\
\itclass~AQLM & 6 & $+5.76$ & $+0.73$ & 5/6 \\


==> generated/method_rows.tex <==
\spclass~RTN-opt & W2G128 & 6 & 0.3853 & 0.3847 & $-0.05$ & $[-0.29,+0.19]$ & $-0.2$ \\
\spclass~AWQ & W3G128 & 6 & 0.6053 & 0.6049 & $-0.04$ & $[-0.36,+0.28]$ & $-1.0$ \\
\spclass~GPTQ & W3G128 & 6 & 0.5747 & 0.5770 & $+0.23$ & $[-0.91,+1.37]$ & $+3.4$ \\
\midrule
\itclass~OmniQuant & W2G128 & 5 & 0.4225 & 0.4403 & $+1.78$ & $[+1.28,+2.27]$ & $+8.2$ \\
\itclass~SR-V2 & W2G128 & 6 & 0.5367 & 0.5550 & $+1.83$ & $[+0.91,+2.75]$ & $+17.3$ \\
\itclass~AQLM & W2-equiv. & 6 & 0.5906 & 0.5980 & $+0.73$ & $[-0.14,+1.61]$ & $+14.1$ \\


==> generated/overlap_rows.tex <==
42 & 1 & 1 & 1 & 3 & 2 \\
123 & 0 & 4 & 1 & 7 & 0 \\
456 & 0 & 2 & 1 & 6 & 0 \\
789 & 3 & 3 & 2 & 6 & 0 \\


==> generated/primary_model_rows.tex <==
Llama-2-7B & $-0.12$ & $+1.31$ & $+5.05$ & $-1.19$ \\
Mistral-7B & $+0.21$ & $+2.36$ & $+5.68$ & $+0.52$ \\
Q2.5-7B-Inst & $-0.16$ & $+0.54$ & $+0.71$ & $+0.47$ \\
Qwen3-1.7B & $-0.35$ & $+2.31$ & $+5.13$ & $+0.75$ \\
Qwen3-8B & $+0.23$ & $+1.50$ & $+2.72$ & $+0.46$ \\


==> generated/random_qa_rows.tex <==
Llama-2-7B & $+1.91$ & $+0.92$ \\
Mistral-7B & $+3.45$ & $+2.86$ \\
Q2.5-7B-Inst & $-0.86$ & $+0.41$ \\
Qwen3-1.7B & $+1.37$ & $+2.85$ \\
Qwen3-8B & $+0.03$ & $+1.59$ \\
Phi-3-mini & $+2.84$ & $+2.97$ \\


==> generated/regime_rows.tex <==
W2G128 & Llama-2-7B & 0.295$^\dagger$ & 0.319$^\dagger$ & 0.382 & 0.522 & 0.568 \\
W2G128 & Mistral-7B & 0.299$^\dagger$ & 0.310$^\dagger$ & 0.320$^\dagger$ & 0.565 & 0.625 \\
W2G128 & Phi-3-mini & 0.317$^\dagger$ & 0.299$^\dagger$ & 0.390 & 0.525 & 0.624 \\
W2G128 & Q2.5-7B-Inst & 0.298$^\dagger$ & 0.313$^\dagger$ & 0.515 & 0.602 & 0.595 \\
W2G128 & Qwen3-1.7B & 0.320$^\dagger$ & 0.305$^\dagger$ & 0.366 & 0.435 & 0.503 \\
W2G128 & Qwen3-8B & 0.321$^\dagger$ & 0.317$^\dagger$ & 0.460 & 0.571 & 0.630 \\
W3G128 & Llama-2-7B & 0.582 & 0.574 & 0.580 & 0.584 & --- \\
W3G128 & Mistral-7B & 0.637 & 0.619 & 0.625 & 0.645 & --- \\
W3G128 & Phi-3-mini & 0.633 & 0.579 & 0.619 & 0.646 & --- \\
W3G128 & Q2.5-7B-Inst & 0.663 & 0.631 & 0.661 & 0.672 & --- \\
W3G128 & Qwen3-1.7B & 0.490 & 0.447 & 0.516 & 0.532 & --- \\
W3G128 & Qwen3-8B & 0.627 & 0.597 & 0.631 & 0.652 & --- \\


==> generated/same_w3_rows.tex <==
Llama-2-7B & $+0.77$ \\
Mistral-7B & $+0.52$ \\
Phi-3-mini-4k-instruct & $-0.24$ \\
Q2.5-7B-Inst & $-0.01$ \\
Qwen3-1.7B & $+0.48$ \\
Qwen3-8B & $-1.17$ \\


==> generated/seed_rows.tex <==
\spclass~RTN-opt & Llama-2-7B & 42 & 0.4130 & 0.4125 & $-0.04$ \\
\spclass~RTN-opt & Llama-2-7B & 123 & 0.4150 & 0.4130 & $-0.20$ \\
\spclass~RTN-opt & Llama-2-7B & 456 & 0.4112 & 0.4101 & $-0.11$ \\
\spclass~RTN-opt & Llama-2-7B & 789 & 0.4129 & 0.4118 & $-0.11$ \\
\spclass~RTN-opt & Mistral-7B & 42 & 0.4467 & 0.4515 & $+0.48$ \\
\spclass~RTN-opt & Mistral-7B & 123 & 0.4474 & 0.4490 & $+0.16$ \\
\spclass~RTN-opt & Mistral-7B & 456 & 0.4253 & 0.4269 & $+0.16$ \\
\spclass~RTN-opt & Mistral-7B & 789 & 0.4499 & 0.4503 & $+0.04$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & 42 & 0.3666 & 0.3679 & $+0.12$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & 123 & 0.3742 & 0.3665 & $-0.77$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & 456 & 0.3701 & 0.3728 & $+0.27$ \\
\spclass~RTN-opt & Q2.5-7B-Inst & 789 & 0.3714 & 0.3688 & $-0.26$ \\
\spclass~RTN-opt & Qwen3-1.7B & 42 & 0.3131 & 0.3075 & $-0.57$ \\
\spclass~RTN-opt & Qwen3-1.7B & 123 & 0.3099 & 0.3046 & $-0.54$ \\
\spclass~RTN-opt & Qwen3-1.7B & 456 & 0.3081 & 0.3072 & $-0.09$ \\
\spclass~RTN-opt & Qwen3-1.7B & 789 & 0.3109 & 0.3087 & $-0.21$ \\
\spclass~RTN-opt & Qwen3-8B & 42 & 0.3850 & 0.3872 & $+0.21$ \\
\spclass~RTN-opt & Qwen3-8B & 123 & 0.3858 & 0.3913 & $+0.55$ \\
\spclass~RTN-opt & Qwen3-8B & 456 & 0.3875 & 0.3894 & $+0.19$ \\
\spclass~RTN-opt & Qwen3-8B & 789 & 0.3885 & 0.3881 & $-0.04$ \\
\itclass~SR-V2 & Llama-2-7B & 42 & 0.5212 & 0.5355 & $+1.43$ \\
\itclass~SR-V2 & Llama-2-7B & 123 & 0.5207 & 0.5353 & $+1.46$ \\
\itclass~SR-V2 & Llama-2-7B & 456 & 0.5264 & 0.5404 & $+1.39$ \\
\itclass~SR-V2 & Llama-2-7B & 789 & 0.5213 & 0.5308 & $+0.95$ \\
\itclass~SR-V2 & Mistral-7B & 42 & 0.5643 & 0.5869 & $+2.26$ \\
\itclass~SR-V2 & Mistral-7B & 123 & 0.5662 & 0.5876 & $+2.15$ \\
\itclass~SR-V2 & Mistral-7B & 456 & 0.5671 & 0.5948 & $+2.76$ \\
\itclass~SR-V2 & Mistral-7B & 789 & 0.5635 & 0.5863 & $+2.28$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & 42 & 0.5968 & 0.6075 & $+1.07$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & 123 & 0.6051 & 0.6078 & $+0.26$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & 456 & 0.6065 & 0.6075 & $+0.09$ \\
\itclass~SR-V2 & Q2.5-7B-Inst & 789 & 0.5987 & 0.6060 & $+0.73$ \\
\itclass~SR-V2 & Qwen3-1.7B & 42 & 0.4370 & 0.4552 & $+1.82$ \\
\itclass~SR-V2 & Qwen3-1.7B & 123 & 0.4345 & 0.4593 & $+2.48$ \\
\itclass~SR-V2 & Qwen3-1.7B & 456 & 0.4331 & 0.4622 & $+2.91$ \\
\itclass~SR-V2 & Qwen3-1.7B & 789 & 0.4349 & 0.4552 & $+2.04$ \\
\itclass~SR-V2 & Qwen3-8B & 42 & 0.5701 & 0.5865 & $+1.64$ \\
\itclass~SR-V2 & Qwen3-8B & 123 & 0.5757 & 0.5867 & $+1.10$ \\
\itclass~SR-V2 & Qwen3-8B & 456 & 0.5665 & 0.5865 & $+2.00$ \\
\itclass~SR-V2 & Qwen3-8B & 789 & 0.5708 & 0.5834 & $+1.26$ \\


==> generated/targeting_rows.tex <==
Fragility-selected tasks & $+3.86$ & $[+1.25,+6.46]$ & 5/5 \\
Strict non-targeted tasks & $+0.20$ & $[-0.78,+1.18]$ & 4/5 \\
Within-model difference & $+3.65$ & $[+0.67,+6.64]$ & 5/5 \\


==> generated/transfer_rows.tex <==
Llama-2-7B & $+3.08$ & 4/4 \\
Mistral-7B & $+0.37$ & 3/4 \\
Qwen2.5-7B-Instruct & $+1.10$ & 4/4 \\
Qwen3-1.7B & $+2.05$ & 4/4 \\
Qwen3-8B & $+0.93$ & 4/4 \\


==> generated/width_rows.tex <==
\spclass~RTN-opt & Single-pass & $-0.05$ & $-0.2$ & $-0.02$ & $-0.4$ & $-0.02$ & $-2.2$ \\
\spclass~AWQ & Single-pass & $+0.02$ & $+0.0$ & $-0.04$ & $-1.0$ & $-0.03$ & $-4.4$ \\
\spclass~GPTQ & Single-pass & $-0.44$ & $-1.3$ & $+0.23$ & $+3.4$ & $-0.07$ & $-5.7$ \\
\midrule
\itclass~OmniQuant & Iterative & $+1.78$ & $+8.2$ & $-0.05$ & $-1.4$ & $-0.08$ & $-9.7$ \\
\itclass~SR-V2 & Iterative & $+1.83$ & $+17.3$ & $+0.36$ & $+17.3$ & $+0.01$ & $+2.4$ \\
\itclass~AQLM & Iterative & $+0.73$ & $+14.1$ & --- & --- & --- & --- \\


==> generated/wikitext_proxy_rows.tex <==
Llama-2-7B & $-0.00138$ & $+1.31$ \\
Mistral-7B & $+0.04614$ & $+2.36$ \\
Q2.5-7B-Inst & $+0.00333$ & $+0.54$ \\
Qwen3-1.7B & $+0.11028$ & $+2.31$ \\
Qwen3-8B & $+0.03733$ & $+1.50$ \\

